XOOD: Extreme Value Based Out-Of-Distribution Detection For Image Classification

Detecting out-of-distribution (OOD) data at inference time is crucial for many applications of machine learning. We present XOOD: a novel extreme value-based OOD detection framework for image classification that consists of two algorithms. The first, XOOD-M, is completely unsupervised, while the second XOOD-L is self-supervised. Both algorithms rely on the signals captured by the extreme values of the data in the activation layers of the neural network in order to distinguish between in-distribution and OOD instances. We show experimentally that both XOOD-M and XOOD-L outperform state-of-the-art OOD detection methods on many benchmark data sets in both efficiency and accuracy, reducing false-positive rate (FPR95) by 50%, while improving the inferencing time by an order of magnitude.

==> XOOD Preprint/feature_addition.tex <==
\begin{table}[H]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllllllllll}
\toprule
{} & \multicolumn{4}{l}{cifar10} & \multicolumn{4}{l}{svhn} & \multicolumn{4}{l}{cifar100} \\
{} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} \\
{} &         \texttt{XOOD-M} &              \texttt{XOOD-L} &         \texttt{XOOD-M} &             \texttt{XOOD-L} &         \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &         \texttt{XOOD-M} &              \texttt{XOOD-L} \\
\midrule
Min \& Max  &  \textbf{99.7} &           99.46 &  \textbf{99.4} &  \textbf{99.5} &          99.77 &           99.85 &           99.94 &           99.97 &  \textbf{98.42} &            97.8 &  \textbf{97.3} &  \textbf{98.18} \\
Positivity &          99.68 &  \textbf{99.54} &          99.27 &          99.34 &          99.88 &           99.92 &  \textbf{99.95} &  \textbf{99.98} &           98.14 &           97.21 &           97.0 &           97.52 \\
Sum        &          99.64 &            99.5 &          99.28 &          99.19 &  \textbf{99.9} &  \textbf{99.93} &           99.94 &           99.96 &           98.22 &           97.66 &          96.85 &           97.45 \\
L1         &          99.62 &           99.43 &          99.33 &          99.38 &          99.79 &           99.87 &           99.93 &           99.92 &            98.3 &            97.5 &          96.63 &           97.74 \\
L2         &          99.63 &           99.42 &          99.37 &          99.39 &          99.79 &           99.78 &           99.94 &           99.92 &           98.18 &           97.61 &          96.69 &           97.86 \\
L3         &          99.63 &           99.43 &          99.39 &          99.39 &           99.8 &           99.78 &           99.94 &           99.93 &           98.18 &           97.58 &          96.76 &           97.97 \\
Split L1   &          99.57 &           99.43 &          99.26 &          99.17 &           99.9 &           99.91 &           99.93 &           99.95 &           98.21 &            97.5 &          96.33 &           97.11 \\
Split L2   &          99.59 &           99.41 &          99.29 &          99.22 &          99.86 &           99.87 &           99.94 &           99.94 &           98.13 &           97.82 &          96.28 &           97.51 \\
Split L3   &          99.62 &           99.44 &          99.33 &          99.25 &          99.87 &           99.87 &           99.93 &           99.94 &           98.21 &  \textbf{97.85} &          96.36 &           97.74 \\
\bottomrule
\end{tabular}
}
    \caption{AUROC-score when extracting additional extreme values before each activation layer.}
    \label{Table: Feature Addition}
\end{table}



==> XOOD Preprint/feature_selection.tex <==
\begin{table}[H]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllllllllll}
\toprule
{} & \multicolumn{4}{l}{cifar10} & \multicolumn{4}{l}{svhn} & \multicolumn{4}{l}{cifar100} \\
{} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} & \multicolumn{2}{l}{resnet} & \multicolumn{2}{l}{densenet} \\
{} &         \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} &          \texttt{XOOD-M} &              \texttt{XOOD-L} \\
\midrule
Min \& Max  &  \textbf{99.7} &  \textbf{99.47} &            99.4 &  \textbf{99.55} &  \textbf{99.77} &  \textbf{99.85} &  \textbf{99.94} &  \textbf{99.97} &  \textbf{98.42} &           97.86 &            97.3 &  \textbf{98.29} \\
Min        &          99.63 &            99.4 &           99.23 &           99.41 &           99.43 &           99.77 &           99.87 &           99.93 &           98.17 &  \textbf{98.04} &           96.63 &           96.84 \\
Max        &          99.59 &           99.32 &  \textbf{99.43} &           99.54 &            99.6 &           99.69 &           99.91 &           99.97 &            97.4 &           97.13 &  \textbf{97.37} &           97.48 \\
Positivity &          97.86 &           98.76 &           95.56 &           98.22 &           99.43 &           99.82 &           99.45 &           99.81 &           89.76 &           90.47 &           91.38 &           92.06 \\
Sum        &          97.67 &           98.92 &           96.06 &            97.1 &           99.54 &           99.81 &           99.64 &           99.75 &            92.2 &           96.41 &           92.32 &           92.82 \\
L1         &          98.15 &           98.75 &           98.11 &            98.2 &           98.87 &           99.53 &           99.69 &           99.74 &           93.55 &           95.77 &           92.22 &           94.18 \\
L2         &           98.5 &           98.78 &           98.57 &           98.68 &           98.98 &           99.51 &           99.78 &           99.82 &           93.71 &           96.01 &           93.19 &           94.78 \\
L3         &          98.83 &            98.9 &           98.83 &           98.99 &           99.16 &           99.54 &            99.8 &           99.87 &           94.74 &           95.96 &           94.01 &           95.37 \\
Split L1   &          98.59 &           98.96 &            98.2 &           98.19 &           99.69 &           99.78 &           99.82 &           99.88 &           95.36 &           96.23 &           93.03 &           93.13 \\
Split L2   &          98.94 &           99.08 &           98.61 &           98.89 &           99.61 &           99.72 &           99.86 &           99.89 &           95.94 &           97.36 &            93.6 &           94.74 \\
Split L3   &          99.23 &           99.18 &           98.92 &           99.24 &           99.69 &           99.82 &           99.88 &           99.92 &            96.8 &            97.5 &           94.33 &           95.66 \\
\bottomrule
\end{tabular}
}
    \caption{AUROC-score when replacing the extreme values with other features which have linear computational complexity.}
    \label{Table: Feature Selection}
\end{table}



==> XOOD Preprint/fpr_table.tex <==
\begin{table}[H]
    \centering
    \begin{tabular}{lrrrrrr}
        & Baseline & ODIN & Mahalanobis & Gram & XOOD-L & XOOD-M \\
        \hline
        ResNet34 & 55.7	& 37.6 & 8.6& 7.1& 5.2 & 3.5 \\
        DenseNet & 51.8	& 28.4 & 15.2 & 6.9 & 3.6 & 5.1\\
    \end{tabular}
    \caption{Average FPR at 95\% TPR. Lower score is better.}
    \label{fpr-table}
\end{table}

==> XOOD Preprint/gram_table.tex <==
\begin{table}[ht]
\caption{\textbf{DenseNet} detection scores for Baseline/Odin/Mahalanobis/Gram/XOOD-L/XOOD-M. Results for other algorithms are from  Sastry and Oore \cite{gram}.} \label{Table:DenseNet}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccc}
\toprule
     &      &                                    TNR (95\% TPR) &                                                     AUROC &                                   Detection Acc. \\
In Dist & Out Dist &                                                  &                                                           &                                                  \\
\midrule
CIFAR-10 & CIFAR-100 &           40.3/\textbf{53.1}/14.5/26.7/47.6/19.9 &                    89.3/\textbf{90.2}/58.5/72.0/87.0/70.7 &           \textbf{82.9}/82.7/57.2/67.3/78.6/64.8 \\
     & LSUN-C &           51.8/70.6/48.2/88.4/\textbf{96.9}/91.7 &                    92.9/93.6/80.2/97.5/\textbf{99.3}/98.4 &           86.9/86.4/75.6/92.0/\textbf{96.1}/93.6 \\
     & LSUN-R &           66.6/96.2/97.2/99.5/99.4/\textbf{99.7} &  95.4/99.2/99.3/\textbf{99.9}/\textbf{99.9}/\textbf{99.9} &  90.3/95.7/96.3/\textbf{98.6}/98.5/\textbf{98.6} \\
     & SVHN &           40.2/86.2/90.8/96.1/96.5/\textbf{97.2} &                    89.9/95.5/98.1/99.1/99.2/\textbf{99.3} &           83.2/91.4/93.9/95.9/96.2/\textbf{96.7} \\
     & TinyImgNet-C &           56.7/87.0/84.2/96.7/\textbf{98.6}/97.8 &                    93.8/97.6/95.3/99.3/\textbf{99.7}/99.5 &           88.1/92.3/89.9/96.1/\textbf{97.7}/96.6 \\
     & TinyImgNet-R &           58.9/92.4/95.0/98.8/99.1/\textbf{99.2} &           94.1/98.5/98.8/99.7/\textbf{99.8}/\textbf{99.8} &           88.5/93.9/95.0/97.9/\textbf{98.2}/97.8 \\
     & iSUN &           62.5/93.2/95.3/99.0/\textbf{99.5}/99.4 &                    94.7/98.7/98.9/99.8/\textbf{99.9}/99.8 &           89.2/94.3/95.2/97.9/\textbf{98.5}/98.1 \\
CIFAR-100 & CIFAR-10 &           \textbf{18.9}/16.8/ 7.7/10.6/10.0/ 1.7 &                    \textbf{75.9}/74.2/60.1/64.2/65.0/43.1 &           \textbf{69.7}/68.6/57.8/60.4/61.8/50.0 \\
     & LSUN-C &           28.6/57.8/42.1/65.5/\textbf{84.9}/68.4 &                    80.2/91.4/81.7/91.4/\textbf{97.4}/92.6 &           72.7/83.3/74.0/83.6/\textbf{91.3}/85.0 \\
     & LSUN-R &           17.6/41.2/91.4/97.2/94.3/\textbf{97.9} &           70.8/85.5/98.0/\textbf{99.3}/99.0/\textbf{99.3} &           64.9/77.1/93.9/96.4/94.8/\textbf{96.7} \\
     & SVHN &           26.7/70.6/82.5/\textbf{89.3}/88.8/87.9 &                    82.7/93.8/97.2/97.3/\textbf{97.7}/97.1 &           75.6/86.6/91.5/\textbf{92.4}/92.3/91.9 \\
     & TinyImgNet-C &           24.6/51.0/60.1/89.0/\textbf{95.4}/89.2 &                    76.2/88.3/88.8/97.7/\textbf{99.1}/97.5 &           69.0/80.2/81.6/92.5/\textbf{95.2}/92.7 \\
     & TinyImgNet-R &           17.6/42.6/86.6/95.7/95.7/\textbf{96.1} &                    71.7/85.2/97.4/99.0/\textbf{99.2}/98.9 &           65.7/77.0/92.2/95.5/95.4/\textbf{95.6} \\
     & iSUN &           14.9/37.4/87.0/95.9/94.0/\textbf{96.3} &           69.5/84.5/97.4/\textbf{99.0}/98.9/\textbf{99.0} &           63.8/76.4/92.4/95.6/94.6/\textbf{95.7} \\
SVHN & CIFAR-10 &           69.3/71.7/96.8/80.4/\textbf{99.7}/98.4 &                    91.9/91.4/98.9/95.5/\textbf{99.8}/99.5 &           86.6/85.8/95.9/89.1/\textbf{98.3}/97.0 \\
     & LSUN-R &  77.1/81.1/99.9/99.5/\textbf{100.}/\textbf{100.} &           94.1/94.5/99.9/99.8/\textbf{100.}/\textbf{100.} &  89.1/89.2/99.3/98.6/\textbf{99.8}/\textbf{99.8} \\
     & TinyImgNet-R &  79.8/84.1/99.9/99.1/\textbf{100.}/\textbf{100.} &           94.8/95.1/99.9/99.7/\textbf{100.}/\textbf{100.} &           90.2/90.4/98.9/97.9/99.5/\textbf{99.6} \\
     & iSUN &  78.3/82.2/99.9/99.4/\textbf{100.}/\textbf{100.} &           94.4/94.7/99.9/99.8/\textbf{100.}/\textbf{100.} &           89.6/89.7/99.2/98.3/99.7/\textbf{99.8} \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[ht]
\caption{\textbf{ResNet34} detection scores for Baseline/Odin/Mahalanobis/Gram/XOOD-L/XOOD-M. Results for other algorithms are from  Sastry and Oore \cite{gram}.} \label{Table:ResNet}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccc}
\toprule
     &      &                                    TNR (95\% TPR) &                                                     AUROC &                          Detection Acc. \\
In Dist & Out Dist &                                                  &                                                           &                                         \\
\midrule
CIFAR-10 & CIFAR-100 &           33.3/42.0/41.6/32.9/\textbf{43.6}/32.0 &                    86.4/85.8/88.2/79.0/\textbf{88.8}/80.1 &  80.4/78.6/81.2/71.7/\textbf{81.7}/73.7 \\
     & LSUN-C &           48.6/62.0/81.3/89.8/\textbf{97.0}/94.6 &                    91.9/91.2/96.7/97.8/\textbf{99.4}/99.0 &  86.3/82.4/90.5/92.6/\textbf{96.0}/94.8 \\
     & LSUN-R &           49.8/82.1/98.8/99.6/99.1/\textbf{99.9} &                    91.0/94.1/99.7/99.9/99.8/\textbf{100.} &  85.3/86.7/97.7/98.6/97.8/\textbf{99.2} \\
     & SVHN &           50.5/70.3/87.8/97.6/96.4/\textbf{98.4} &                    89.9/96.7/99.1/99.5/99.3/\textbf{99.7} &  85.1/91.1/95.8/96.7/96.1/\textbf{97.6} \\
     & TinyImgNet-C &           46.4/68.7/92.0/96.7/98.0/\textbf{99.1} &                    91.4/93.1/98.6/99.2/99.5/\textbf{99.8} &  85.4/85.2/93.9/96.1/96.7/\textbf{98.0} \\
     & TinyImgNet-R &           41.0/67.9/97.1/98.7/97.9/\textbf{99.5} &                    91.0/94.0/99.5/99.7/99.6/\textbf{99.9} &  85.1/86.5/96.3/97.8/96.9/\textbf{98.8} \\
     & iSUN &           44.6/73.2/97.8/99.3/99.1/\textbf{99.7} &                    91.0/94.0/99.5/99.8/99.8/\textbf{99.9} &  85.0/86.5/96.7/98.1/97.8/\textbf{98.8} \\
CIFAR-100 & CIFAR-10 &           19.1/18.7/\textbf{20.2}/12.2/11.7/ 9.3 &                    77.1/77.2/\textbf{77.5}/67.9/71.0/63.9 &  71.0/71.2/\textbf{72.1}/63.4/67.1/61.6 \\
     & LSUN-C &           18.7/44.1/64.8/64.8/\textbf{85.3}/76.2 &                    75.5/82.7/92.0/92.1/\textbf{97.5}/95.3 &  69.2/75.9/84.0/84.2/\textbf{91.4}/88.2 \\
     & LSUN-R &           18.8/23.2/90.9/96.6/90.2/\textbf{98.5} &                    75.8/85.6/98.2/99.2/98.3/\textbf{99.6} &  69.9/78.3/93.5/96.7/92.9/\textbf{97.4} \\
     & SVHN &           20.3/62.7/91.9/80.8/87.2/\textbf{92.1} &                    79.5/93.9/\textbf{98.4}/96.0/97.6/98.2 &  73.2/88.0/\textbf{93.7}/89.6/91.5/93.6 \\
     & TinyImgNet-C &           24.3/44.3/80.9/88.5/90.8/\textbf{95.0} &                    79.7/85.4/96.3/97.7/98.4/\textbf{98.9} &  72.5/78.3/89.9/92.2/93.2/\textbf{95.0} \\
     & TinyImgNet-R &           20.4/36.1/90.9/94.8/89.4/\textbf{97.9} &                    77.2/87.6/98.2/98.9/98.1/\textbf{99.5} &  70.8/80.1/93.3/95.0/92.6/\textbf{96.7} \\
     & iSUN &           16.9/45.2/89.9/94.8/89.6/\textbf{97.0} &                    75.8/85.5/97.9/98.8/98.3/\textbf{99.3} &  70.1/78.5/93.1/95.6/92.8/\textbf{96.2} \\
SVHN & CIFAR-10 &           78.3/79.8/\textbf{98.4}/85.8/98.1/96.1 &                    92.9/92.1/99.3/97.3/\textbf{99.5}/98.9 &  90.0/89.4/\textbf{96.9}/92.0/96.8/95.7 \\
     & LSUN-R &  74.3/77.3/\textbf{99.9}/99.6/99.5/\textbf{99.9} &  91.6/89.4/\textbf{99.9}/99.8/\textbf{99.9}/\textbf{99.9} &  89.0/87.2/\textbf{99.5}/98.5/98.3/98.9 \\
     & TinyImgNet-R &           79.0/82.0/\textbf{99.9}/99.3/99.7/99.8 &           93.5/92.0/\textbf{99.9}/99.7/\textbf{99.9}/99.8 &  90.4/89.4/\textbf{99.1}/97.9/98.4/98.6 \\
     & iSUN &           77.1/79.1/99.7/99.4/99.8/\textbf{99.9} &           92.2/91.4/99.8/99.8/\textbf{99.9}/\textbf{99.9} &  89.7/89.2/98.3/98.1/98.7/\textbf{98.9} \\
\bottomrule
\end{tabular}
}
\end{table}


==> XOOD Preprint/new_react_table.tex <==
\begin{table}[H]
\caption{Baseline/Energy/React/XOOD-L/XOOD-M.}
\resizebox{\textwidth}{!}{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tabular}{llllll}
\toprule
         &          &      &                                                 TNR (95\% TPR) &                              Detection Acc. &                                       AUROC \\
\midrule
imagenet & resnet18 & Uniform &   2.5/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &           86.9/99.1/99.7/\textbf{100.}/99.9 &  86.9/99.7/99.9/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/80.4/72.1/\textbf{100.}/\textbf{100.} &           76.0/95.3/94.4/\textbf{100.}/99.9 &  65.1/96.2/95.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             23.9/34.8/\textbf{57.2}/37.1/34.2 &           70.7/75.9/\textbf{82.3}/76.7/70.7 &           78.0/83.6/\textbf{89.7}/84.4/77.1 \\
         &          & SUN &                             26.4/40.0/\textbf{65.5}/46.9/48.6 &           71.6/78.4/\textbf{85.3}/79.9/77.9 &           78.9/86.1/\textbf{92.7}/88.0/85.2 \\
         &          & iNaturalist &                             41.6/43.2/\textbf{69.9}/60.9/38.9 &           78.9/82.5/\textbf{87.4}/84.8/74.4 &           87.0/89.8/\textbf{94.6}/92.8/82.0 \\
         &          & DTD &                             28.6/46.7/60.8/56.9/\textbf{61.8} &           71.3/79.1/\textbf{83.6}/81.4/81.8 &           78.4/86.3/\textbf{91.4}/88.9/89.5 \\
         & resnet34 & Uniform &           86.4/\textbf{100.}/99.6/\textbf{100.}/\textbf{100.} &  94.6/98.1/97.3/\textbf{100.}/\textbf{100.} &  97.2/98.7/98.4/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    48.6/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  92.5/89.8/89.1/\textbf{100.}/\textbf{100.} &  94.3/85.9/85.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             26.1/37.2/\textbf{64.1}/38.6/34.2 &           71.4/77.0/\textbf{84.2}/77.8/69.8 &           79.2/84.6/\textbf{91.4}/85.6/75.9 \\
         &          & SUN &                             27.6/42.6/\textbf{73.6}/48.4/48.1 &           72.3/79.2/\textbf{87.5}/81.0/76.9 &           79.8/86.6/\textbf{94.0}/88.6/83.8 \\
         &          & iNaturalist &                             40.5/46.0/\textbf{75.9}/65.1/40.2 &           78.3/82.2/\textbf{88.8}/86.1/74.1 &           86.6/89.7/\textbf{95.7}/93.7/81.5 \\
         &          & DTD &                             29.9/44.9/55.3/61.5/\textbf{70.5} &           71.7/79.3/83.5/83.7/\textbf{85.1} &           79.1/86.5/91.2/91.0/\textbf{92.4} \\
         & resnet50 & Uniform &   3.6/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &  89.7/98.3/99.6/\textbf{100.}/\textbf{100.} &  89.8/98.9/99.8/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  69.7/81.6/87.6/\textbf{100.}/\textbf{100.} &  53.2/75.5/85.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.0/34.8/\textbf{66.6}/43.5/32.0 &           72.8/76.9/\textbf{85.0}/79.6/69.9 &           80.6/84.2/\textbf{92.0}/87.2/75.9 \\
         &          & SUN &                             31.0/41.9/\textbf{76.0}/54.4/47.8 &           74.0/79.4/\textbf{87.9}/82.7/77.6 &           81.7/86.8/\textbf{94.4}/90.4/84.8 \\
         &          & iNaturalist &                             46.8/46.3/\textbf{80.5}/71.2/44.8 &           79.9/83.9/\textbf{90.0}/88.3/76.9 &           88.4/90.7/\textbf{96.4}/95.1/84.6 \\
         &          & DTD &                             33.5/47.9/54.3/64.8/\textbf{71.0} &           73.0/79.7/82.8/84.1/\textbf{85.4} &           80.4/86.8/90.5/91.3/\textbf{92.9} \\
         & resnet101 & Uniform &           27.1/96.7/\textbf{100.}/\textbf{100.}/\textbf{100.} &  87.3/96.5/99.3/\textbf{100.}/\textbf{100.} &  90.8/97.2/99.6/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &            0.0/ 0.0/\textbf{100.}/\textbf{100.}/\textbf{100.} &  79.0/88.0/98.3/\textbf{100.}/\textbf{100.} &  70.6/83.9/98.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.8/39.4/\textbf{63.7}/42.7/26.7 &           72.9/78.2/\textbf{84.2}/79.7/71.2 &           80.6/85.5/\textbf{91.3}/87.2/77.0 \\
         &          & SUN &                             32.1/46.8/\textbf{73.4}/51.0/41.3 &           73.9/80.6/\textbf{87.2}/82.6/78.3 &           81.4/87.7/\textbf{94.0}/89.9/85.2 \\
         &          & iNaturalist &                             42.9/41.6/\textbf{79.1}/61.9/32.5 &           77.4/81.1/\textbf{89.5}/86.3/75.7 &           86.2/88.3/\textbf{96.1}/93.4/82.8 \\
         &          & DTD &                             37.4/52.6/59.6/67.5/\textbf{68.6} &           73.4/80.8/83.5/85.4/\textbf{87.2} &           81.5/87.9/91.4/92.4/\textbf{94.0} \\
cifar10 & resnet & Uniform &                    72.7/82.0/90.2/\textbf{100.}/\textbf{100.} &  93.6/94.2/94.6/\textbf{100.}/\textbf{100.} &  96.1/96.2/96.8/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    90.8/98.8/98.1/\textbf{100.}/\textbf{100.} &  95.7/97.0/96.6/\textbf{100.}/\textbf{100.} &  97.5/98.0/98.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                             46.9/62.1/65.1/98.0/\textbf{99.1} &           85.5/86.5/86.5/96.7/\textbf{98.0} &           91.6/93.1/92.6/99.5/\textbf{99.8} \\
         &          & TinyImageNet (Resize) &                             45.1/59.5/63.9/97.9/\textbf{99.5} &           85.1/85.8/86.3/96.9/\textbf{98.8} &           91.1/92.5/92.4/99.6/\textbf{99.9} \\
         &          & LSUN (Crop) &                             49.1/65.7/62.5/\textbf{97.0}/94.6 &           86.4/87.5/85.1/\textbf{96.0}/94.8 &           92.0/93.9/90.9/\textbf{99.4}/99.0 \\
         &          & LSUN (Resize) &                             46.3/62.9/69.4/99.1/\textbf{99.9} &           85.5/86.7/88.2/97.8/\textbf{99.2} &           91.3/92.9/94.4/99.8/\textbf{100.} \\
         &          & iSUN &                             45.6/62.0/68.0/99.1/\textbf{99.7} &           85.2/86.3/87.9/97.8/\textbf{98.8} &           91.2/92.8/94.2/99.8/\textbf{99.9} \\
         &          & SVHN &                             33.3/47.9/37.9/96.4/\textbf{98.4} &           85.4/85.5/77.5/96.1/\textbf{97.6} &           90.1/91.3/83.3/99.3/\textbf{99.7} \\
         &          & Cifar100 &                    34.2/\textbf{44.0}/\textbf{44.0}/43.6/32.0 &           80.5/80.7/78.7/\textbf{81.7}/73.7 &           86.6/87.3/84.4/\textbf{88.8}/80.1 \\
         & densenet & Uniform &           78.0/96.7/\textbf{100.}/\textbf{100.}/\textbf{100.} &  94.8/96.3/98.1/\textbf{100.}/\textbf{100.} &  96.7/97.4/99.2/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &  89.3/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &  95.4/97.9/98.4/\textbf{100.}/\textbf{100.} &  97.7/98.9/99.5/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                             57.4/84.1/68.6/\textbf{98.6}/97.8 &           88.2/91.6/87.6/\textbf{97.7}/96.6 &           94.0/97.1/94.1/\textbf{99.7}/99.5 \\
         &          & TinyImageNet (Resize) &                             60.1/86.2/68.7/99.1/\textbf{99.2} &           88.8/92.3/87.3/\textbf{98.2}/97.8 &  94.3/97.5/94.0/\textbf{99.8}/\textbf{99.8} \\
         &          & LSUN (Crop) &                             52.4/76.1/66.4/\textbf{96.9}/91.7 &           87.2/89.8/88.4/\textbf{96.1}/93.6 &           93.2/96.0/94.4/\textbf{99.3}/98.4 \\
         &          & LSUN (Resize) &                             67.3/92.3/83.1/99.4/\textbf{99.7} &           90.5/93.9/91.4/98.5/\textbf{98.6} &  95.6/98.4/96.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             63.8/89.3/78.4/\textbf{99.5}/99.4 &           89.5/93.1/90.0/\textbf{98.5}/98.1 &           95.0/98.0/96.1/\textbf{99.9}/99.8 \\
         &          & SVHN &                             40.9/52.9/65.3/96.5/\textbf{97.2} &           83.4/83.5/88.1/96.2/\textbf{96.7} &           90.1/91.1/93.8/99.2/\textbf{99.3} \\
         &          & Cifar100 &                             41.7/\textbf{55.3}/49.3/47.6/19.9 &           83.2/\textbf{83.6}/82.2/78.6/64.8 &           89.6/\textbf{90.7}/89.2/87.0/70.7 \\
svhn & resnet & Uniform &                    85.9/86.7/71.9/\textbf{100.}/\textbf{100.} &           93.0/92.5/84.7/99.5/\textbf{99.7} &  96.1/95.6/89.4/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    86.1/87.3/75.2/\textbf{100.}/\textbf{100.} &           93.0/92.7/86.1/99.7/\textbf{99.9} &  96.3/96.0/90.5/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                    81.3/83.0/74.4/\textbf{99.7}/\textbf{99.7} &           91.1/90.7/85.5/\textbf{98.7}/98.3 &           94.2/93.8/88.7/\textbf{99.9}/99.8 \\
         &          & TinyImageNet (Resize) &                             79.8/81.5/74.1/99.7/\textbf{99.8} &           90.6/90.1/85.2/98.4/\textbf{98.6} &           93.6/93.0/88.9/\textbf{99.9}/99.8 \\
         &          & LSUN (Crop) &                             77.2/79.0/71.5/\textbf{99.2}/98.6 &           89.9/89.4/84.0/\textbf{97.7}/97.0 &           92.9/92.5/86.2/\textbf{99.7}/99.5 \\
         &          & LSUN (Resize) &                             75.5/77.2/67.2/99.5/\textbf{99.9} &           89.1/88.3/82.0/98.3/\textbf{98.9} &  91.6/90.7/84.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             78.1/79.8/69.0/99.8/\textbf{99.9} &           89.9/89.4/82.7/98.7/\textbf{98.9} &  92.3/91.5/85.6/\textbf{99.9}/\textbf{99.9} \\
         &          & Cifar100 &                             77.7/78.9/74.0/\textbf{97.8}/95.5 &           89.5/88.9/85.2/\textbf{96.4}/95.5 &           92.4/91.5/89.1/\textbf{99.3}/98.9 \\
         & densenet & Uniform &                    66.3/64.0/37.9/\textbf{100.}/\textbf{100.} &  87.7/83.6/79.0/\textbf{100.}/\textbf{100.} &  93.2/90.1/87.2/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    88.2/90.8/55.9/\textbf{100.}/\textbf{100.} &  93.5/93.2/84.1/\textbf{100.}/\textbf{100.} &  97.4/97.8/91.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                             79.1/77.1/72.4/\textbf{100.}/99.9 &           89.9/87.4/86.6/\textbf{99.4}/99.3 &  94.7/92.8/93.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Resize) &                    80.1/78.7/73.1/\textbf{100.}/\textbf{100.} &           90.3/88.1/87.0/99.5/\textbf{99.6} &  94.9/93.4/93.5/\textbf{100.}/\textbf{100.} \\
         &          & LSUN (Crop) &                             74.0/67.8/71.6/\textbf{99.7}/99.2 &           88.1/83.2/85.5/\textbf{98.7}/97.8 &           93.0/88.5/92.1/\textbf{99.9}/99.8 \\
         &          & LSUN (Resize) &                    77.4/76.8/70.6/\textbf{100.}/\textbf{100.} &  89.3/87.1/85.4/\textbf{99.8}/\textbf{99.8} &  94.2/92.6/92.3/\textbf{100.}/\textbf{100.} \\
         &          & iSUN &                    78.7/78.2/70.2/\textbf{100.}/\textbf{100.} &           89.8/87.6/85.8/99.7/\textbf{99.8} &  94.5/92.9/92.6/\textbf{100.}/\textbf{100.} \\
         &          & Cifar100 &                             68.5/64.6/74.8/\textbf{98.1}/97.9 &           86.6/83.0/87.3/\textbf{96.8}/96.7 &           91.4/88.2/93.9/\textbf{99.5}/99.4 \\
cifar100 & resnet & Uniform &                    12.1/ 1.6/ 1.3/\textbf{100.}/\textbf{100.} &  81.5/84.7/80.6/\textbf{100.}/\textbf{100.} &  85.2/86.5/81.6/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  60.7/60.8/81.7/\textbf{100.}/\textbf{100.} &  45.1/46.1/76.6/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                             25.0/27.1/28.5/90.8/\textbf{95.0} &           72.6/74.4/71.2/93.2/\textbf{95.0} &           79.7/81.6/78.9/98.4/\textbf{98.9} \\
         &          & TinyImageNet (Resize) &                             21.3/25.3/25.6/89.4/\textbf{97.9} &           71.0/73.0/68.6/92.6/\textbf{96.7} &           77.2/80.1/76.2/98.1/\textbf{99.5} \\
         &          & LSUN (Crop) &                             19.2/18.0/28.0/\textbf{85.3}/76.2 &           69.6/69.2/77.7/\textbf{91.4}/88.2 &           75.6/75.1/84.3/\textbf{97.5}/95.3 \\
         &          & LSUN (Resize) &                             19.4/23.3/23.0/90.2/\textbf{98.5} &           70.0/71.9/68.5/92.9/\textbf{97.4} &           75.7/78.5/75.5/98.3/\textbf{99.6} \\
         &          & iSUN &                             17.7/20.9/21.5/89.6/\textbf{97.0} &           70.3/72.1/68.5/92.8/\textbf{96.2} &           75.8/78.2/75.3/98.3/\textbf{99.3} \\
         &          & SVHN &                             21.3/18.8/26.3/87.2/\textbf{92.1} &           73.4/73.5/77.3/91.5/\textbf{93.6} &           79.5/79.5/84.2/97.6/\textbf{98.2} \\
         & densenet & Uniform &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  64.2/66.7/76.1/\textbf{100.}/\textbf{100.} &  43.3/50.3/74.0/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  58.9/53.0/69.8/\textbf{100.}/\textbf{100.} &  30.8/15.6/58.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Crop) &                             23.5/39.3/65.1/\textbf{95.4}/89.2 &           68.8/76.9/86.4/\textbf{95.2}/92.7 &           75.9/84.8/93.7/\textbf{99.1}/97.5 \\
         &          & TinyImageNet (Resize) &                             16.6/22.8/64.4/95.7/\textbf{96.1} &           65.9/71.4/86.8/95.4/\textbf{95.6} &           71.5/78.2/93.8/\textbf{99.2}/98.9 \\
         &          & LSUN (Crop) &                             27.5/51.9/43.8/\textbf{84.9}/68.4 &           72.5/82.2/79.0/\textbf{91.3}/85.0 &           79.8/90.1/87.2/\textbf{97.4}/92.6 \\
         &          & LSUN (Resize) &                             15.8/22.0/72.8/94.3/\textbf{97.9} &           65.0/72.4/88.8/94.8/\textbf{96.7} &           70.6/79.5/95.3/99.0/\textbf{99.3} \\
         &          & iSUN &                             14.2/18.2/68.4/94.0/\textbf{96.3} &           64.0/70.5/86.9/94.6/\textbf{95.7} &           69.5/77.2/93.9/98.9/\textbf{99.0} \\
         &          & SVHN &                             25.2/33.2/33.1/\textbf{88.8}/87.9 &           75.5/80.5/79.5/\textbf{92.3}/91.9 &           82.4/87.7/86.9/\textbf{97.7}/97.1 \\
\bottomrule
\label{reacttable}

\end{tabular}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

}
\end{table}

==> XOOD Preprint/react_table.tex <==
\begin{table}[h]
\caption{Baseline/Energy/React/XOOD-L/XOOD-M.}
\resizebox{\textwidth}{!}{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tabular}{lllccc}
\toprule
         &          &      &                                                 TNR (95\% TPR) &                              Detection Acc. &                                       AUROC \\
\midrule
imagenet & resnet18 & Uniform &   2.5/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &           86.9/99.1/99.7/\textbf{100.}/99.9 &  86.9/99.7/99.9/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/80.4/72.1/\textbf{100.}/\textbf{100.} &           76.0/95.3/94.4/\textbf{100.}/99.9 &  65.1/96.2/95.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             23.9/34.8/\textbf{57.2}/37.1/34.2 &           70.7/75.9/\textbf{82.3}/76.7/70.7 &           78.0/83.6/\textbf{89.7}/84.4/77.1 \\
         &          & SUN &                             26.4/40.0/\textbf{65.5}/46.9/48.6 &           71.6/78.4/\textbf{85.3}/79.9/77.9 &           78.9/86.1/\textbf{92.7}/88.0/85.2 \\
         &          & iNaturalist &                             41.6/43.2/\textbf{69.9}/60.9/38.9 &           78.9/82.5/\textbf{87.4}/84.8/74.4 &           87.0/89.8/\textbf{94.6}/92.8/82.0 \\
         &          & DTD &                             28.6/46.7/60.8/56.9/\textbf{61.8} &           71.3/79.1/\textbf{83.6}/81.4/81.8 &           78.4/86.3/\textbf{91.4}/88.9/89.5 \\
         & resnet34 & Uniform &           86.4/\textbf{100.}/99.6/\textbf{100.}/\textbf{100.} &  94.6/98.1/97.3/\textbf{100.}/\textbf{100.} &  97.2/98.7/98.4/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    48.6/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  92.5/89.8/89.1/\textbf{100.}/\textbf{100.} &  94.3/85.9/85.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             26.1/37.2/\textbf{64.1}/38.6/34.2 &           71.4/77.0/\textbf{84.2}/77.8/69.8 &           79.2/84.6/\textbf{91.4}/85.6/75.9 \\
         &          & SUN &                             27.6/42.6/\textbf{73.6}/48.4/48.1 &           72.3/79.2/\textbf{87.5}/81.0/76.9 &           79.8/86.6/\textbf{94.0}/88.6/83.8 \\
         &          & iNaturalist &                             40.5/46.0/\textbf{75.9}/65.1/40.2 &           78.3/82.2/\textbf{88.8}/86.1/74.1 &           86.6/89.7/\textbf{95.7}/93.7/81.5 \\
         &          & DTD &                             29.9/44.9/55.3/61.5/\textbf{70.5} &           71.7/79.3/83.5/83.7/\textbf{85.1} &           79.1/86.5/91.2/91.0/\textbf{92.4} \\
         & resnet50 & Uniform &   3.6/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &  89.7/98.3/99.6/\textbf{100.}/\textbf{100.} &  89.8/98.9/99.8/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  69.7/81.6/87.6/\textbf{100.}/\textbf{100.} &  53.2/75.5/85.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.0/34.8/\textbf{66.6}/43.5/32.0 &           72.8/76.9/\textbf{85.0}/79.6/69.9 &           80.6/84.2/\textbf{92.0}/87.2/75.9 \\
         &          & SUN &                             31.0/41.9/\textbf{76.0}/54.4/47.8 &           74.0/79.4/\textbf{87.9}/82.7/77.6 &           81.7/86.8/\textbf{94.4}/90.4/84.8 \\
         &          & iNaturalist &                             46.8/46.3/\textbf{80.5}/71.2/44.8 &           79.9/83.9/\textbf{90.0}/88.3/76.9 &           88.4/90.7/\textbf{96.4}/95.1/84.6 \\
         &          & DTD &                             33.5/47.9/54.3/64.8/\textbf{71.0} &           73.0/79.7/82.8/84.1/\textbf{85.4} &           80.4/86.8/90.5/91.3/\textbf{92.9} \\
         & resnet101 & Uniform &           27.1/96.7/\textbf{100.}/\textbf{100.}/\textbf{100.} &  87.3/96.5/99.3/\textbf{100.}/\textbf{100.} &  90.8/97.2/99.6/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &            0.0/ 0.0/\textbf{100.}/\textbf{100.}/\textbf{100.} &  79.0/88.0/98.3/\textbf{100.}/\textbf{100.} &  70.6/83.9/98.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.8/39.4/\textbf{63.7}/42.7/26.7 &           72.9/78.2/\textbf{84.2}/79.7/71.2 &           80.6/85.5/\textbf{91.3}/87.2/77.0 \\
         &          & SUN &                             32.1/46.8/\textbf{73.4}/51.0/41.3 &           73.9/80.6/\textbf{87.2}/82.6/78.3 &           81.4/87.7/\textbf{94.0}/89.9/85.2 \\
         &          & iNaturalist &                             42.9/41.6/\textbf{79.1}/61.9/32.5 &           77.4/81.1/\textbf{89.5}/86.3/75.7 &           86.2/88.3/\textbf{96.1}/93.4/82.8 \\
         &          & DTD &                             37.4/52.6/59.6/67.5/\textbf{68.6} &           73.4/80.8/83.5/85.4/\textbf{87.2} &           81.5/87.9/91.4/92.4/\textbf{94.0} \\
cifar10 & resnet & TinyImageNet (Crop) &                             46.9/62.1/65.1/98.0/\textbf{99.1} &           85.5/86.5/86.5/96.7/\textbf{98.0} &           91.6/93.1/92.6/99.5/\textbf{99.8} \\
         &          & TinyImageNet (Resize) &                             45.1/59.5/63.9/97.9/\textbf{99.5} &           85.1/85.8/86.3/96.9/\textbf{98.8} &           91.1/92.5/92.4/99.6/\textbf{99.9} \\
         &          & LSUN (Crop) &                             49.1/65.7/62.5/\textbf{97.0}/94.6 &           86.4/87.5/85.1/\textbf{96.0}/94.8 &           92.0/93.9/90.9/\textbf{99.4}/99.0 \\
         &          & LSUN (Resize) &                             46.3/62.9/69.4/99.1/\textbf{99.9} &           85.5/86.7/88.2/97.8/\textbf{99.2} &           91.3/92.9/94.4/99.8/\textbf{100.} \\
         &          & iSUN &                             45.6/62.0/68.0/99.1/\textbf{99.7} &           85.2/86.3/87.9/97.8/\textbf{98.8} &           91.2/92.8/94.2/99.8/\textbf{99.9} \\
         &          & SVHN &                             33.3/47.9/37.9/96.4/\textbf{98.4} &           85.4/85.5/77.5/96.1/\textbf{97.6} &           90.1/91.3/83.3/99.3/\textbf{99.7} \\
         &          & Cifar100 &                    34.2/\textbf{44.0}/\textbf{44.0}/43.6/32.0 &           80.5/80.7/78.7/\textbf{81.7}/73.7 &           86.6/87.3/84.4/\textbf{88.8}/80.1 \\
         & densenet & TinyImageNet (Crop) &                             57.4/84.1/68.6/\textbf{98.6}/97.8 &           88.2/91.6/87.6/\textbf{97.7}/96.6 &           94.0/97.1/94.1/\textbf{99.7}/99.5 \\
         &          & TinyImageNet (Resize) &                             60.1/86.2/68.7/99.1/\textbf{99.2} &           88.8/92.3/87.3/\textbf{98.2}/97.8 &  94.3/97.5/94.0/\textbf{99.8}/\textbf{99.8} \\
         &          & LSUN (Crop) &                             52.4/76.1/66.4/\textbf{96.9}/91.7 &           87.2/89.8/88.4/\textbf{96.1}/93.6 &           93.2/96.0/94.4/\textbf{99.3}/98.4 \\
         &          & LSUN (Resize) &                             67.3/92.3/83.1/99.4/\textbf{99.7} &           90.5/93.9/91.4/98.5/\textbf{98.6} &  95.6/98.4/96.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             63.8/89.3/78.4/\textbf{99.5}/99.4 &           89.5/93.1/90.0/\textbf{98.5}/98.1 &           95.0/98.0/96.1/\textbf{99.9}/99.8 \\
         &          & SVHN &                             40.9/52.9/65.3/96.5/\textbf{97.2} &           83.4/83.5/88.1/96.2/\textbf{96.7} &           90.1/91.1/93.8/99.2/\textbf{99.3} \\
         &          & Cifar100 &                             41.7/\textbf{55.3}/49.3/47.6/19.9 &           83.2/\textbf{83.6}/82.2/78.6/64.8 &           89.6/\textbf{90.7}/89.2/87.0/70.7 \\
svhn & resnet & TinyImageNet (Crop) &                    81.3/83.0/74.4/\textbf{99.7}/\textbf{99.7} &           91.1/90.7/85.5/\textbf{98.7}/98.3 &           94.2/93.8/88.7/\textbf{99.9}/99.8 \\
         &          & TinyImageNet (Resize) &                             79.8/81.5/74.1/99.7/\textbf{99.8} &           90.6/90.1/85.2/98.4/\textbf{98.6} &           93.6/93.0/88.9/\textbf{99.9}/99.8 \\
         &          & LSUN (Crop) &                             77.2/79.0/71.5/\textbf{99.2}/98.6 &           89.9/89.4/84.0/\textbf{97.7}/97.0 &           92.9/92.5/86.2/\textbf{99.7}/99.5 \\
         &          & LSUN (Resize) &                             75.5/77.2/67.2/99.5/\textbf{99.9} &           89.1/88.3/82.0/98.3/\textbf{98.9} &  91.6/90.7/84.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             78.1/79.8/69.0/99.8/\textbf{99.9} &           89.9/89.4/82.7/98.7/\textbf{98.9} &  92.3/91.5/85.6/\textbf{99.9}/\textbf{99.9} \\
         &          & Cifar100 &                             77.7/78.9/74.0/\textbf{97.8}/95.5 &           89.5/88.9/85.2/\textbf{96.4}/95.5 &           92.4/91.5/89.1/\textbf{99.3}/98.9 \\
         & densenet & TinyImageNet (Crop) &                             79.1/77.1/72.4/\textbf{100.}/99.9 &           89.9/87.4/86.6/\textbf{99.4}/99.3 &  94.7/92.8/93.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Resize) &                    80.1/78.7/73.1/\textbf{100.}/\textbf{100.} &           90.3/88.1/87.0/99.5/\textbf{99.6} &  94.9/93.4/93.5/\textbf{100.}/\textbf{100.} \\
         &          & LSUN (Crop) &                             74.0/67.8/71.6/\textbf{99.7}/99.2 &           88.1/83.2/85.5/\textbf{98.7}/97.8 &           93.0/88.5/92.1/\textbf{99.9}/99.8 \\
         &          & LSUN (Resize) &                    77.4/76.8/70.6/\textbf{100.}/\textbf{100.} &  89.3/87.1/85.4/\textbf{99.8}/\textbf{99.8} &  94.2/92.6/92.3/\textbf{100.}/\textbf{100.} \\
         &          & iSUN &                    78.7/78.2/70.2/\textbf{100.}/\textbf{100.} &           89.8/87.6/85.8/99.7/\textbf{99.8} &  94.5/92.9/92.6/\textbf{100.}/\textbf{100.} \\
         &          & Cifar100 &                             68.5/64.6/74.8/\textbf{98.1}/97.9 &           86.6/83.0/87.3/\textbf{96.8}/96.7 &           91.4/88.2/93.9/\textbf{99.5}/99.4 \\
cifar100 & resnet & TinyImageNet (Crop) &                             25.0/27.1/28.5/90.8/\textbf{95.0} &           72.6/74.4/71.2/93.2/\textbf{95.0} &           79.7/81.6/78.9/98.4/\textbf{98.9} \\
         &          & TinyImageNet (Resize) &                             21.3/25.3/25.6/89.4/\textbf{97.9} &           71.0/73.0/68.6/92.6/\textbf{96.7} &           77.2/80.1/76.2/98.1/\textbf{99.5} \\
         &          & LSUN (Crop) &                             19.2/18.0/28.0/\textbf{85.3}/76.2 &           69.6/69.2/77.7/\textbf{91.4}/88.2 &           75.6/75.1/84.3/\textbf{97.5}/95.3 \\
         &          & LSUN (Resize) &                             19.4/23.3/23.0/90.2/\textbf{98.5} &           70.0/71.9/68.5/92.9/\textbf{97.4} &           75.7/78.5/75.5/98.3/\textbf{99.6} \\
         &          & iSUN &                             17.7/20.9/21.5/89.6/\textbf{97.0} &           70.3/72.1/68.5/92.8/\textbf{96.2} &           75.8/78.2/75.3/98.3/\textbf{99.3} \\
         &          & SVHN &                             21.3/18.8/26.3/87.2/\textbf{92.1} &           73.4/73.5/77.3/91.5/\textbf{93.6} &           79.5/79.5/84.2/97.6/\textbf{98.2} \\
         & densenet & TinyImageNet (Crop) &                             23.5/39.3/65.1/\textbf{95.4}/89.2 &           68.8/76.9/86.4/\textbf{95.2}/92.7 &           75.9/84.8/93.7/\textbf{99.1}/97.5 \\
         &          & TinyImageNet (Resize) &                             16.6/22.8/64.4/95.7/\textbf{96.1} &           65.9/71.4/86.8/95.4/\textbf{95.6} &           71.5/78.2/93.8/\textbf{99.2}/98.9 \\
         &          & LSUN (Crop) &                             27.5/51.9/43.8/\textbf{84.9}/68.4 &           72.5/82.2/79.0/\textbf{91.3}/85.0 &           79.8/90.1/87.2/\textbf{97.4}/92.6 \\
         &          & LSUN (Resize) &                             15.8/22.0/72.8/94.3/\textbf{97.9} &           65.0/72.4/88.8/94.8/\textbf{96.7} &           70.6/79.5/95.3/99.0/\textbf{99.3} \\
         &          & iSUN &                             14.2/18.2/68.4/94.0/\textbf{96.3} &           64.0/70.5/86.9/94.6/\textbf{95.7} &           69.5/77.2/93.9/98.9/\textbf{99.0} \\
         &          & SVHN &                             25.2/33.2/33.1/\textbf{88.8}/87.9 &           75.5/80.5/79.5/\textbf{92.3}/91.9 &           82.4/87.7/86.9/\textbf{97.7}/97.1 \\
\bottomrule
\label{reacttable}
\end{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

}
\end{table}

==> react_table.tex <==
\begin{table}[h]
\caption{Baseline/Energy/React/XOOD-L/XOOD-M.}
\resizebox{\textwidth}{!}{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tabular}{lllccc}
\toprule
         &          &      &                                                 TNR (95\% TPR) &                              Detection Acc. &                                       AUROC \\
\midrule
imagenet & resnet18 & Uniform &   2.5/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &           86.9/99.1/99.7/\textbf{100.}/99.9 &  86.9/99.7/99.9/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/80.4/72.1/\textbf{100.}/\textbf{100.} &           76.0/95.3/94.4/\textbf{100.}/99.9 &  65.1/96.2/95.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             23.9/34.8/\textbf{57.2}/37.1/34.2 &           70.7/75.9/\textbf{82.3}/76.7/70.7 &           78.0/83.6/\textbf{89.7}/84.4/77.1 \\
         &          & SUN &                             26.4/40.0/\textbf{65.5}/46.9/48.6 &           71.6/78.4/\textbf{85.3}/79.9/77.9 &           78.9/86.1/\textbf{92.7}/88.0/85.2 \\
         &          & iNaturalist &                             41.6/43.2/\textbf{69.9}/60.9/38.9 &           78.9/82.5/\textbf{87.4}/84.8/74.4 &           87.0/89.8/\textbf{94.6}/92.8/82.0 \\
         &          & DTD &                             28.6/46.7/60.8/56.9/\textbf{61.8} &           71.3/79.1/\textbf{83.6}/81.4/81.8 &           78.4/86.3/\textbf{91.4}/88.9/89.5 \\
         & resnet34 & Uniform &           86.4/\textbf{100.}/99.6/\textbf{100.}/\textbf{100.} &  94.6/98.1/97.3/\textbf{100.}/\textbf{100.} &  97.2/98.7/98.4/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                    48.6/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  92.5/89.8/89.1/\textbf{100.}/\textbf{100.} &  94.3/85.9/85.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             26.1/37.2/\textbf{64.1}/38.6/34.2 &           71.4/77.0/\textbf{84.2}/77.8/69.8 &           79.2/84.6/\textbf{91.4}/85.6/75.9 \\
         &          & SUN &                             27.6/42.6/\textbf{73.6}/48.4/48.1 &           72.3/79.2/\textbf{87.5}/81.0/76.9 &           79.8/86.6/\textbf{94.0}/88.6/83.8 \\
         &          & iNaturalist &                             40.5/46.0/\textbf{75.9}/65.1/40.2 &           78.3/82.2/\textbf{88.8}/86.1/74.1 &           86.6/89.7/\textbf{95.7}/93.7/81.5 \\
         &          & DTD &                             29.9/44.9/55.3/61.5/\textbf{70.5} &           71.7/79.3/83.5/83.7/\textbf{85.1} &           79.1/86.5/91.2/91.0/\textbf{92.4} \\
         & resnet50 & Uniform &   3.6/\textbf{100.}/\textbf{100.}/\textbf{100.}/\textbf{100.} &  89.7/98.3/99.6/\textbf{100.}/\textbf{100.} &  89.8/98.9/99.8/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &                     0.0/ 0.0/ 0.0/\textbf{100.}/\textbf{100.} &  69.7/81.6/87.6/\textbf{100.}/\textbf{100.} &  53.2/75.5/85.8/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.0/34.8/\textbf{66.6}/43.5/32.0 &           72.8/76.9/\textbf{85.0}/79.6/69.9 &           80.6/84.2/\textbf{92.0}/87.2/75.9 \\
         &          & SUN &                             31.0/41.9/\textbf{76.0}/54.4/47.8 &           74.0/79.4/\textbf{87.9}/82.7/77.6 &           81.7/86.8/\textbf{94.4}/90.4/84.8 \\
         &          & iNaturalist &                             46.8/46.3/\textbf{80.5}/71.2/44.8 &           79.9/83.9/\textbf{90.0}/88.3/76.9 &           88.4/90.7/\textbf{96.4}/95.1/84.6 \\
         &          & DTD &                             33.5/47.9/54.3/64.8/\textbf{71.0} &           73.0/79.7/82.8/84.1/\textbf{85.4} &           80.4/86.8/90.5/91.3/\textbf{92.9} \\
         & resnet101 & Uniform &           27.1/96.7/\textbf{100.}/\textbf{100.}/\textbf{100.} &  87.3/96.5/99.3/\textbf{100.}/\textbf{100.} &  90.8/97.2/99.6/\textbf{100.}/\textbf{100.} \\
         &          & Gaussian &            0.0/ 0.0/\textbf{100.}/\textbf{100.}/\textbf{100.} &  79.0/88.0/98.3/\textbf{100.}/\textbf{100.} &  70.6/83.9/98.2/\textbf{100.}/\textbf{100.} \\
         &          & Places &                             28.8/39.4/\textbf{63.7}/42.7/26.7 &           72.9/78.2/\textbf{84.2}/79.7/71.2 &           80.6/85.5/\textbf{91.3}/87.2/77.0 \\
         &          & SUN &                             32.1/46.8/\textbf{73.4}/51.0/41.3 &           73.9/80.6/\textbf{87.2}/82.6/78.3 &           81.4/87.7/\textbf{94.0}/89.9/85.2 \\
         &          & iNaturalist &                             42.9/41.6/\textbf{79.1}/61.9/32.5 &           77.4/81.1/\textbf{89.5}/86.3/75.7 &           86.2/88.3/\textbf{96.1}/93.4/82.8 \\
         &          & DTD &                             37.4/52.6/59.6/67.5/\textbf{68.6} &           73.4/80.8/83.5/85.4/\textbf{87.2} &           81.5/87.9/91.4/92.4/\textbf{94.0} \\
cifar10 & resnet & TinyImageNet (Crop) &                             46.9/62.1/65.1/98.0/\textbf{99.1} &           85.5/86.5/86.5/96.7/\textbf{98.0} &           91.6/93.1/92.6/99.5/\textbf{99.8} \\
         &          & TinyImageNet (Resize) &                             45.1/59.5/63.9/97.9/\textbf{99.5} &           85.1/85.8/86.3/96.9/\textbf{98.8} &           91.1/92.5/92.4/99.6/\textbf{99.9} \\
         &          & LSUN (Crop) &                             49.1/65.7/62.5/\textbf{97.0}/94.6 &           86.4/87.5/85.1/\textbf{96.0}/94.8 &           92.0/93.9/90.9/\textbf{99.4}/99.0 \\
         &          & LSUN (Resize) &                             46.3/62.9/69.4/99.1/\textbf{99.9} &           85.5/86.7/88.2/97.8/\textbf{99.2} &           91.3/92.9/94.4/99.8/\textbf{100.} \\
         &          & iSUN &                             45.6/62.0/68.0/99.1/\textbf{99.7} &           85.2/86.3/87.9/97.8/\textbf{98.8} &           91.2/92.8/94.2/99.8/\textbf{99.9} \\
         &          & SVHN &                             33.3/47.9/37.9/96.4/\textbf{98.4} &           85.4/85.5/77.5/96.1/\textbf{97.6} &           90.1/91.3/83.3/99.3/\textbf{99.7} \\
         &          & Cifar100 &                    34.2/\textbf{44.0}/\textbf{44.0}/43.6/32.0 &           80.5/80.7/78.7/\textbf{81.7}/73.7 &           86.6/87.3/84.4/\textbf{88.8}/80.1 \\
         & densenet & TinyImageNet (Crop) &                             57.4/84.1/68.6/\textbf{98.6}/97.8 &           88.2/91.6/87.6/\textbf{97.7}/96.6 &           94.0/97.1/94.1/\textbf{99.7}/99.5 \\
         &          & TinyImageNet (Resize) &                             60.1/86.2/68.7/99.1/\textbf{99.2} &           88.8/92.3/87.3/\textbf{98.2}/97.8 &  94.3/97.5/94.0/\textbf{99.8}/\textbf{99.8} \\
         &          & LSUN (Crop) &                             52.4/76.1/66.4/\textbf{96.9}/91.7 &           87.2/89.8/88.4/\textbf{96.1}/93.6 &           93.2/96.0/94.4/\textbf{99.3}/98.4 \\
         &          & LSUN (Resize) &                             67.3/92.3/83.1/99.4/\textbf{99.7} &           90.5/93.9/91.4/98.5/\textbf{98.6} &  95.6/98.4/96.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             63.8/89.3/78.4/\textbf{99.5}/99.4 &           89.5/93.1/90.0/\textbf{98.5}/98.1 &           95.0/98.0/96.1/\textbf{99.9}/99.8 \\
         &          & SVHN &                             40.9/52.9/65.3/96.5/\textbf{97.2} &           83.4/83.5/88.1/96.2/\textbf{96.7} &           90.1/91.1/93.8/99.2/\textbf{99.3} \\
         &          & Cifar100 &                             41.7/\textbf{55.3}/49.3/47.6/19.9 &           83.2/\textbf{83.6}/82.2/78.6/64.8 &           89.6/\textbf{90.7}/89.2/87.0/70.7 \\
svhn & resnet & TinyImageNet (Crop) &                    81.3/83.0/74.4/\textbf{99.7}/\textbf{99.7} &           91.1/90.7/85.5/\textbf{98.7}/98.3 &           94.2/93.8/88.7/\textbf{99.9}/99.8 \\
         &          & TinyImageNet (Resize) &                             79.8/81.5/74.1/99.7/\textbf{99.8} &           90.6/90.1/85.2/98.4/\textbf{98.6} &           93.6/93.0/88.9/\textbf{99.9}/99.8 \\
         &          & LSUN (Crop) &                             77.2/79.0/71.5/\textbf{99.2}/98.6 &           89.9/89.4/84.0/\textbf{97.7}/97.0 &           92.9/92.5/86.2/\textbf{99.7}/99.5 \\
         &          & LSUN (Resize) &                             75.5/77.2/67.2/99.5/\textbf{99.9} &           89.1/88.3/82.0/98.3/\textbf{98.9} &  91.6/90.7/84.9/\textbf{99.9}/\textbf{99.9} \\
         &          & iSUN &                             78.1/79.8/69.0/99.8/\textbf{99.9} &           89.9/89.4/82.7/98.7/\textbf{98.9} &  92.3/91.5/85.6/\textbf{99.9}/\textbf{99.9} \\
         &          & Cifar100 &                             77.7/78.9/74.0/\textbf{97.8}/95.5 &           89.5/88.9/85.2/\textbf{96.4}/95.5 &           92.4/91.5/89.1/\textbf{99.3}/98.9 \\
         & densenet & TinyImageNet (Crop) &                             79.1/77.1/72.4/\textbf{100.}/99.9 &           89.9/87.4/86.6/\textbf{99.4}/99.3 &  94.7/92.8/93.2/\textbf{100.}/\textbf{100.} \\
         &          & TinyImageNet (Resize) &                    80.1/78.7/73.1/\textbf{100.}/\textbf{100.} &           90.3/88.1/87.0/99.5/\textbf{99.6} &  94.9/93.4/93.5/\textbf{100.}/\textbf{100.} \\
         &          & LSUN (Crop) &                             74.0/67.8/71.6/\textbf{99.7}/99.2 &           88.1/83.2/85.5/\textbf{98.7}/97.8 &           93.0/88.5/92.1/\textbf{99.9}/99.8 \\
         &          & LSUN (Resize) &                    77.4/76.8/70.6/\textbf{100.}/\textbf{100.} &  89.3/87.1/85.4/\textbf{99.8}/\textbf{99.8} &  94.2/92.6/92.3/\textbf{100.}/\textbf{100.} \\
         &          & iSUN &                    78.7/78.2/70.2/\textbf{100.}/\textbf{100.} &           89.8/87.6/85.8/99.7/\textbf{99.8} &  94.5/92.9/92.6/\textbf{100.}/\textbf{100.} \\
         &          & Cifar100 &                             68.5/64.6/74.8/\textbf{98.1}/97.9 &           86.6/83.0/87.3/\textbf{96.8}/96.7 &           91.4/88.2/93.9/\textbf{99.5}/99.4 \\
cifar100 & resnet & TinyImageNet (Crop) &                             25.0/27.1/28.5/90.8/\textbf{95.0} &           72.6/74.4/71.2/93.2/\textbf{95.0} &           79.7/81.6/78.9/98.4/\textbf{98.9} \\
         &          & TinyImageNet (Resize) &                             21.3/25.3/25.6/89.4/\textbf{97.9} &           71.0/73.0/68.6/92.6/\textbf{96.7} &           77.2/80.1/76.2/98.1/\textbf{99.5} \\
         &          & LSUN (Crop) &                             19.2/18.0/28.0/\textbf{85.3}/76.2 &           69.6/69.2/77.7/\textbf{91.4}/88.2 &           75.6/75.1/84.3/\textbf{97.5}/95.3 \\
         &          & LSUN (Resize) &                             19.4/23.3/23.0/90.2/\textbf{98.5} &           70.0/71.9/68.5/92.9/\textbf{97.4} &           75.7/78.5/75.5/98.3/\textbf{99.6} \\
         &          & iSUN &                             17.7/20.9/21.5/89.6/\textbf{97.0} &           70.3/72.1/68.5/92.8/\textbf{96.2} &           75.8/78.2/75.3/98.3/\textbf{99.3} \\
         &          & SVHN &                             21.3/18.8/26.3/87.2/\textbf{92.1} &           73.4/73.5/77.3/91.5/\textbf{93.6} &           79.5/79.5/84.2/97.6/\textbf{98.2} \\
         & densenet & TinyImageNet (Crop) &                             23.5/39.3/65.1/\textbf{95.4}/89.2 &           68.8/76.9/86.4/\textbf{95.2}/92.7 &           75.9/84.8/93.7/\textbf{99.1}/97.5 \\
         &          & TinyImageNet (Resize) &                             16.6/22.8/64.4/95.7/\textbf{96.1} &           65.9/71.4/86.8/95.4/\textbf{95.6} &           71.5/78.2/93.8/\textbf{99.2}/98.9 \\
         &          & LSUN (Crop) &                             27.5/51.9/43.8/\textbf{84.9}/68.4 &           72.5/82.2/79.0/\textbf{91.3}/85.0 &           79.8/90.1/87.2/\textbf{97.4}/92.6 \\
         &          & LSUN (Resize) &                             15.8/22.0/72.8/94.3/\textbf{97.9} &           65.0/72.4/88.8/94.8/\textbf{96.7} &           70.6/79.5/95.3/99.0/\textbf{99.3} \\
         &          & iSUN &                             14.2/18.2/68.4/94.0/\textbf{96.3} &           64.0/70.5/86.9/94.6/\textbf{95.7} &           69.5/77.2/93.9/98.9/\textbf{99.0} \\
         &          & SVHN &                             25.2/33.2/33.1/\textbf{88.8}/87.9 &           75.5/80.5/79.5/\textbf{92.3}/91.9 &           82.4/87.7/86.9/\textbf{97.7}/97.1 \\
\bottomrule
\label{reacttable}
\end{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

}
\end{table}
